Adaptive Learning Material Recommendation in Online Language Education

Recommending personalized learning materials for online language learning is challenging because we typically lack data about the student's ability and the relative difficulty of learning materials. This makes it hard to recommend appropriate content that matches the student's prior knowledge. In this paper, we propose a refined hierarchical knowledge structure to model vocabulary knowledge, which enables us to automatically organize the authentic and up-to-date learning materials collected from the internet. Based on this knowledge structure, we then introduce a hybrid approach to recommend learning materials that adapts to a student's language level. We evaluate our work with an online Japanese learning tool and the results suggest adding adaptivity into material recommendation significantly increases student engagement.

==> JRec_old.tex <==
%\input{fig-jrec}

\section{Evaluation of Adaptive Recommendation}
We evaluate our adaptive learning material recommender system in \emph{JRec}, a Japanese reading text recommendation tool. Our corpus of 380 articles was collected from NHK Easy~\cite{website:nhkeasy}, a Japanese news website for language learners. In order to accommodate beginners, our tool split those articles into 4,267 sentences and paragraphs such that students do not have to read the whole article. Afterwards, it analyzed the hierarchical structure of vocabulary knowledge in the corpus and built a fuzzy partial ordering graph. When using this tool, users are directed to an NHK Easy webpage, read a recommended text (a paragraph or a sentence), and respond whether or not they understand it. Our tool highlights the recommended text and grays out the rest of the webpage. Figure~\ref{fig:jrec} shows a screenshot of JRec.
We released our tool in the Japanese Learning Sub-reddit~\cite{website:reddit} and recruited \japaneseparticipants~users in three days.

%Many users commented that they really needed such a material recommendation tool for language learning: \emph{``I always have a hard time finding just the right books to read.''} \emph{``I'd be very happy to have some recommended texts that are close to my level because reading superconductivity textbooks through a dictionary can get tiring.''} Some users even hoped that we would incorporate more corpora: \emph{``Try adding web novels. They are a good source of intermediate/advanced texts and are also free.''}



\subsection{Adding Adaptivity Improved Engagement Significantly}



In JRec, we tested two different versions of our recommendation algorithm: the adaptive version and the non-adaptive version. The adaptive version includes recommendation and adaptive assessment, and as we discussed in the last section, assessment and recommendation are balanced by the probabilistic heuristic. The non-adaptive version only provides ZPD-based recommendations and does not include adaptive assessment. Both versions start from an assumption of no prior knowledge. We wanted to see whether the adaptive version is more engaging than the non-adaptive version. If this is the case, then this result will validate that incorporating adaptive assessment can enhance recommendation.

%\input{fig-jrec_results}

In order to measure student engagement in our tool, we recorded the number of texts each user read before leaving. In our experiment, 115 randomly selected users used the adaptive recommendation and 91 users used the non-adaptive recommendation\footnote{Users were randomly and evenly distributed into the two conditions, but the tool only recorded when users responded to a text. Two groups had unbalanced number of users because more people quit in the non-adaptive group after reading the first text before responding to it.}.  Since our data was not normally distributed, we used the Wilcoxon-Kruskal-Wallis test.
We observed that the median users in the adaptive group~($Median=12$) read 50\% more texts than those in the non-adaptive group~($Median=8$), and the difference between the two groups was statistically significant~($p=.022$, $r=.16$). Figure~\ref{fig:jrec_results} shows the proportions of users remaining after reading certain amounts of texts. It is clear that adaptive recommendation led users to read more texts before leaving than the non-adaptive version. This result demonstrates that the hybrid approach balancing adaptive assessment and recommendation (adaptive group) is much more engaging than recommendation alone (non-adaptive group), which suggests that adding adaptivity can significantly enhance learning material recommendation in online learning.
\input{fig-combined_2}

==> Multimedia.tex <==

\section{Multimedia Learning Materials}

%Chalenges of education without multimedia(why multimedia)
%Language education using not only texts, but audio. 
%To do this, we want to extend to ....multimedia in the same po graph. 
%In order to further leverage online content for language learning, we would like to extend our language tutoring system to incorporate video/audio learning materials in additional to texts. This will not only increase the abundance of the corpus, but improve the student's learning experiences in multiple aspects. First, some students may favor visual learning style over verbal learning style \cite{} and a multimedia tutoring system can better accommodate them. Also, some topics are much better presented in form of audio or video, such as ``how to make a phone call'' (better learned by audios) and  ``how to buy groceries''(better learned by videos), and a multimedia tutoring system can help students grow language skills in a wider range of practical scenarios.
%Furthermore, incorporating multimedia materials increases the variability of the learn ing process. Students are less likely to get bored of repetitive and similar content and potentially get more engaged,  if the tutoring system alternatively recommends textual, audio and video materials to them.

Contemporary language education utilizes not only texts, but also audios and videos as learning content. There are multiple reasons to incorporate multimedia materials in language learning. First, some students may favor visual or oral content over textual content, and we need to prepare various types of materials to accommodate their preferences. Also, there are topics in language learning that are much better presented in the form of audio or video, such as ``how to make a phone call'' and  ``how to buy groceries'', thus adding audio and video materials can help students grow language skills in a wider range of practical scenarios. Furthermore, incorporating multimedia materials increases the variability of the learning process. Students are less likely to get bored of repetitive and similar content and potentially get more engaged,  if the tutoring system alternately recommends textual, audio and video materials to them.


Therefore, we want to build a multimedia language tutoring system that can prepare curricula containing all three types of media: texts, audios and videos. This is complicated because materials of different media contain different set of language knowledge. Some knowledge is shared among materials of different media while others are distinct. For example, vocabulary knowledge is shared by all three media, pronunciation knowledge is shared by audio and video, and subtitles can only be found in videos. Ideally, the tutoring system would be able to organize both the common and distinct language skills among multimedia materials within the same model, such that the assessment of common language skills can be shared, and the tutoring system can move back and forth between distinct language skills across multimedia materials.





To this end, we extend our fuzzy partial ordering graph to model multimedia learning materials within the same hierarchical knowledge structure. Like we discussed in Section 3, our model evaluates the difficulty of a text based on its vocabulary words. For audio and video materials, our system considered two additional features to determine their difficulties. Given two audio/video materials with the same set of vocabulary, we hypothesize that the audio/video that speaks faster tends to be harder to understand. We also believe that videos without subtitles are also harder than those with subtitles attached. Therefore, we model the language knowledge within multimedia materials with different sets of features:
\begin{itemize}
    \item texts are modeled only by their vocabulary words,
    \item audios are modeled by vocabulary words and speaking rate, and 
    \item videos are modeled by vocabulary words, speaking rate and whether it has subtitles.
\end{itemize}
Here the speaking rate needs to be measured carefully since different languages may have different metrics. Our work focuses on Japanese language learning and we use ``number of \emph{moras}~\cite{otake1993mora} per second'' as the metric of speaking rate in Japanese. 




Now we can extend our fuzzy partial ordering graph to model the hierarchical knowledge structure of our multimedia corpus: each node represents a text, audio or video learning material and there is an edge between one node to another if the first material is $\alpha$-fuzzily directly harder than the second material. We use speaking rate and subtitle features in addition to vocabulary words to specify ``harder-than'' relations for audios and videos: for two audios, we compare their vocabulary (whether one covers at least a proportion of $\alpha$ of vocabulary of the other, see Definition~\ref{def:fuzzy}), speaking rate and whether they have subtitles; for audio/audio or audio/video pairs, we compare their vocabulary and speaking rate; for text/text, text/audio or text/video pairs, we only consider vocabulary words to judge whether one is fuzzily harder than the other.




\input{fig-multimedia_fuzzypo_edgenum}

\input{fig-multimedia_pograph}


We implemented our fuzzy partial ordering graph in a multimedia corpus. Our corpus consists of 20 audios, 18 videos and 38 texts, totalling 76 materials. Audio and video materials were collected from \emph{Easy Japanese}~\cite{website:easyjapanese}, \emph{News in slow Japanese}~\cite{website:newsinslowjapanese}, \emph{the Japanese Page}~\cite{website:thejapanesepage} and YouTube. Text materials were selected from our NHK easy corpus, which we have used in Section 5. We illustrate a sample fuzzy partial ordering graph of our multimedia corpus in Figure~\ref{fig:multimedia_pograph}. The fuzzy partial ordering graph evaluates the relative difficulty of two materials of same or different media within the same hierarchical structure, which enables us to prepare a sequence of multimedia content with gradually increasing difficulty, such that students can experience text, audio and video materials alternately. For example,
one possible sequence of multimedia materials (from easy to hard) in Figure~\ref{fig:multimedia_pograph} can be \emph{Video 23, Text 59, Audio 19, Audio 17}.

As we discussed in section 3, the (fuzzy) partial ordering graph needs to be sufficiently dense so that it can be useful in material recommendation. To further study the graph density, we studied the number of edges (namely, number of ``harder than'' relations between two materials in our multimedia corpus) over different fuzzy parameters and present the results in Figure~\ref{fig:multimedia_fuzzypo_edgenum}. Similar to the results in Figure~\ref{fig:fuzzy_density}, the number of edges increases exponentially as the fuzzy parameter drops. As we discussed in section 3, decreasing the fuzzy parameter will reduce our confidence in the fuzzy partial orderings. Therefore, we need to select a good fuzzy parameter in order to have enough fuzzy partial ordering edges in the hierarchical knowledge structure while ensuring the confidence in those fuzzy partial orderings is still acceptably high.

Apart from tuning the fuzzy parameter, we also found that a good selection of multimedia materials could improve the density of the fuzzy partial ordering graph. We noticed that video materials are usually informal, and most of them are dialogues, whereas text materials are relative formal, using more advanced vocabulary words. The gap of degree of formality may  have restricted the number of partial ordering relations between materials of different media. To bridge this gap, we selected shorter, easier and informal texts to build our multimedia corpus. By doing this, we got roughly 20\% more edges than the initial, randomly selected corpus. In short, materials of difference media need to have similar difficulties, such that students can frequently move back and forth among materials of three different media in order to learn and reinforce different language skills in various scenarios.


In conclusion, using fuzzy partial ordering graphs, we are able to automatically model the difficulties of multimedia materials within the same hierarchical structure. This will enable us to build an online tutoring system that alternately recommends multimedia materials to students, so as to help them grow language skills in a wider range of scenarios.



==> alg-scale_progression.tex <==
\begin{algorithm}
\caption{Scaling a reinforcement-free progression into a longer and slower progression according to parameter $minR$}
\label{alg:scale_progression}
\begin{algorithmic}[1]
\REQUIRE{\ \ reinforcement-free progression $P_0$ and \\\ \ \ \ \ \ \ \ minimum memory retention parameter $minR$}
\ENSURE{longer and slower progression $P$}
\STATE{\textbf{Initialization}:\ \ $P\gets[]$,\ \ $pointer\gets 1$} \label{alg:line:init}
\WHILE{ $pointer \leq \text{length of }P_0$ }
\STATE{$s\gets$ the problem in $P$ with the least memory retention}
\IF{ $P\ne[]$\ \AND\ $\text{memory retention of }s < minR$ } \label{alg:line:judge}
\STATE{Append $s$ to $P$} \label{alg:line:reinforce}
\ELSE
\STATE{Append $P_0[pointer]$ to $P$, $pointer\gets pointer+1$} \label{alg:line:introduce}
\ENDIF
\STATE{Update memory retention for all problems in $P$} \label{alg:line:update}
\ENDWHILE
\STATE{\textbf{return} target progression $P$}
\end{algorithmic}  
\end{algorithm}


==> fig-combined_1.tex <==
\begin{figure}[t]
    \minipage{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/pograph_cropped.pdf}
        %\vspace{0.1in}
        \caption{A sample partial ordering graph. Each node represents a practice problem containing a specific set of required concepts. Directed edges represent a ``directly harder than'' relation between two nodes.}
        \label{fig:po_graph}
    \endminipage
    \hfill
    \minipage{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/fuzzypo_edgenum.pdf}
        \vspace{-0.3in}
        \caption{Number of edges in the fuzzy partial ordering graph over different fuzzy parameters, in our corpus of 4,269 texts. Decreasing the fuzzy parameter will increase the graph density exponentially.}
        \label{fig:fuzzy_density}
    \endminipage
    \vspace{-.14in}
\end{figure}

==> fig-combined_2.tex <==
\begin{figure}[t]
    \minipage{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/JRec.pdf}
        \caption{Screenshot of \emph{JRec}, a Japanese reading text recommendation tool. When using this tool, users are directed to an NHK Easy webpage~\cite{website:nhkeasy}, read a recommended text, and respond whether or not they understand it. Our tool highlights the recommended text and grays out the rest of the webpage.}
        %\vspace{-0.1in}
        \label{fig:jrec}
    \endminipage
    \hfill
    \iffalse
    \minipage{0.48\textwidth}
        \vspace{-0.15in}
        \includegraphics[width=\textwidth]{images/num_texts_read_curve.pdf}
        \vspace{-0.15in}        
        \caption{Proportion of users remaining after reading certain amount of texts. We observed that users in the adaptive group read 62.5\% more texts than those in the non-adaptive group, which indicates that incorporating adaptive assessment significantly improved student engagement in learning material recommendation.}
        \label{fig:jrec_results}
    \endminipage
    \fi
    \minipage{0.48\textwidth}
    \centering
    \begin{tabular}{|c|c|}
    \hline
    Comparison & Results\\
    \hline
    A.R. vs N.R. & $p = .035, Z = 2.109$\\
    A.O. vs A.R. & $p = .766, Z = 0.298$\\
    A.O. vs N.R. & $p = .022, Z = 2.287$\\
    Rand vs N.R. & $p = .547, Z = 0.603$\\
    A.O. vs Rand & $p = .294, Z = 1.049$\\
    A.R. vs Rand & $p = .389, Z = 0.861$\\
    \hline
    \end{tabular}
    \captionof{table}{We ran Wilcoxon Rank-sum tests for all pairs of our four groups: Adaptive Recommendation~(A.R.), Non-adaptive Recommendation~(N.R.), Assessment-Only~(A.O.) and Random~(Rand.). The difference between adaptive recommendation and non-adaptive recommendation was statistically significant~($p=.035$).}   
    \label{tab:jrec_stats}
    \endminipage
\end{figure}

==> fig-jrec.tex <==
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{images/JRec.pdf}
\caption{Screenshot of \emph{JRec}, a Japanese reading text recommendation tool. When using this tool, users are directed to an NHK Easy webpage, read a recommended text, and respond whether or not they understand it. Our tool highlights the recommended text and grays out the rest of the webpage.}
\label{fig:jrec}
\end{figure}

==> fig-jrec_results.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{images/num_texts_read_curve.pdf}
\caption{Proportions of users remaining after reading certain amounts of texts in \emph{JRec}. We observed that users in the adaptive group read more texts than those in the non-adaptive group, which indicates that incorporating adaptive assessment significantly improved student engagement in learning material recommendation.}
\label{fig:jrec_results}
%\vspace{-0.1in}
\end{figure}

==> fig-jrec_results_two.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/num_texts_read_curve.pdf}
        \subcaption{Proportions of users remaining after reading certain amounts of texts.}
        \label{fig:jrec_num_texts}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/total_read_time_curve.pdf}
        \subcaption{Proportions of users remaining after using our tool for certain amounts of time.}
        \label{fig:jrec_time}
    \end{minipage}
\vspace{0.1in}
\caption{User evaluation of JRec, our material recommendation tool. We observed that users in the adaptive group read more texts and used our tool for more time, compared to those in the non-adaptive group, which indicates that incorporating adaptive assessment significantly improved student engagement in learning material recommendation.}
\label{fig:jrec_results}
\end{figure*}

==> fig-multimedia_fuzzypo_edgenum.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.46\textwidth]{images/multimedia_fuzzypo_edgenum_cropped.pdf}
\caption{Number of edges in the fuzzy partial ordering graph over different fuzzy parameters, in our multimedia corpus of 20 audios, 18 videos and 38 texts. The graph density increases exponentially as the fuzzy parameter drops.}
\label{fig:multimedia_fuzzypo_edgenum}
\vspace{-0.15in}
\end{figure*}

% alpha

==> fig-multimedia_pograph.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.90\textwidth]{images/fuzzypo_multimedia_cropped.pdf}
\caption{A subgraph of the fuzzy partial ordering graph for our multimedia corpus. Orange/green/blue nodes represent audio/text/video materials, and each edge represents a ``directly harder than'' relation between two materials of same or different media. Our corpus consists of 20 audios~(labeled from 1 to 20), 18 videos~(labeled from 21 to 38) and 38 texts~(labeled from 39 to 76). We evaluate the difficulties of texts based on vocabulary, audios based on vocabulary and speaking rate, and videos based on vocabulary, speaking rate and whether they have subtitles. We use different features to determine whether there is a ``harder than'' relation between two materials. For two videos, we compare vocabulary, speaking rate and whether they have subtitles; for audio/audio or audio/video pairs, we compare vocabulary and speaking rate; for text/text, text/audio or text/video pairs, we only compare their vocabulary.}
\label{fig:multimedia_pograph}
\end{figure*}


% large arrow
% different arrow color + legend
% other arrows go non-node

==> fig-num_texts_read_bar.tex <==
\begin{figure}
\centering
\includegraphics[width=0.46\textwidth]{images/num_texts_read_bar.pdf}
\caption{Number of texts read by users in two conditions: adaptive recommendation and non-adaptive recommendation.}
\label{fig:num_texts_read_bar}
\end{figure}

==> fig-num_texts_read_curve.tex <==
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{images/num_texts_read_curve.pdf}
\caption{Proportion of users remaining after reading certain amount of texts. We observed that users in the adaptive group read 46\% more texts than those in the non-adaptive group, which indicates that incorporating adaptive assessment significantly improved student engagement in learning material recommendation.}
\label{fig:num_texts_read_curve}
\end{figure}

==> student_modeling.tex <==
\section{Modeling Students' Learning Preferences}

==> tab-fuzzy_examples2.tex <==
\begin{CJK}{UTF8}{min}
\renewcommand{\arraystretch}{1.35}
\begin{table*}%[!b]
\centering
\begin{tabular}{|c|l|}
\hline
$\alpha$ & \multicolumn{1}{|c|}{ Sample Sentence Pair}\\
\hline\hline
\multirow{4}{*}{0.9} & {\footnotesize 席の数より客のほうが多かったことは、５回ありました。}\\ 
\multirow{4}{*}{}    & {\footnotesize ``There were 5 times when there were more passengers than the number of seats.''}\\\cline{2-2}
\multirow{4}{*}{}    & {\footnotesize 先月、全日空の飛行機が、席の数より客が１人多いまま出発しようとしたことがありました。}\\
\multirow{4}{*}{}    & {\footnotesize ``Last month, there was a time when an ANA flight was about to depart, there was one more passenger than the number of seats.''}\\
\hline\hline
\multirow{4}{*}{0.8} & {\footnotesize ９日、このボランティアになりたい人たちが集まって、太田市で勉強しました。}\\
\multirow{4}{*}{}    & {\footnotesize  ``On the 9th, people who wanted to become volunteers gathered and studied in Ota.''}\\ \cline{2-2}
\multirow{4}{*}{}    & {\footnotesize 集まった人たちは、あと２回勉強してテストに合格すると、病院などで通訳をするボランティアになります。}\\
\multirow{4}{*}{}    & {\footnotesize ``The gathered people will become interpretation volunteers in places like hospitals, if they study two more times and pass the test.''}\\ 
\hline\hline
\multirow{4}{*}{0.7} & {\footnotesize シリアでは、政府と政府に反対する人たちの戦争が続いています。}\\ 
\multirow{4}{*}{}    & {\footnotesize ``In Syria, the war between the government and the anti-government faction is still ongoing.''}\\\cline{2-2}
\multirow{4}{*}{}    & {\footnotesize 政府に反対する人たちがたくさんいるアレッポという町には、政府の軍が２週間も空から攻撃を続けています。}\\
\multirow{4}{*}{}    & {\footnotesize ``In Aleppo, where there is a large anti-government faction, the government army maintained attacks from the air for two weeks.''}\\
\hline\hline
\multirow{4}{*}{0.6} & {\footnotesize シリアでは、政府と政府に反対する人たちの戦争が続いています。}\\ 
\multirow{4}{*}{}    & {\footnotesize ``In Syria, the war between the government and the anti-government faction is still ongoing.''}\\\cline{2-2}
\multirow{4}{*}{}    & {\footnotesize 今までの１０年、私は戦争が続いている所や難民が生活している所へ何度も行きました。}\\
\multirow{4}{*}{}    & {\footnotesize ``In the last 10 years, I have made multiple visits to places where a war was ongoing or refugees were living.''}\\
\hline
\end{tabular}
\caption{Sample Sentence Pairs in Fuzzy Partial Ordering. For each fuzzy parameter $\alpha$, the second sentence is $\alpha$-fuzzily harder than the first sentence. As the fuzzy parameter $\alpha$ decreases, the fuzzy partial ordering confidence (the likelihood for a student understand the first sentence, if he/she understands the second one) also drops.  Text source: NHK Easy.}
\label{tab:fuzzy_pair}
\end{table*}
\end{CJK}

==> tab-fuzzy_examples3.tex <==
\begin{table*}
\scriptsize{
\begin{CJK}{UTF8}{min}

\begin{exe}
%{\small\exi{$\alpha$} \textbf{Sample Sentence Pair}}
\exi{\textbf{0.9}}
%\ex
\gll 席   の 数     より 客        のほうが 多かった ことは、 ５回      ありました\\ 
     seat of number than passenger {}        more    {}       {5 times} {there was}\\
\glt \textbf{``There were 5 times when there were more passengers than the number of seats.''}\\
\vspace{-0.05in}
\gll 先月、 全日空 の 飛行機 が、 席 の 数 より 客 が １人 多い まま 出発しよう としたことが ありました\\
    {last month} ANA of {flight} {} seat of number than passenger {} {1 person} {more} {} {about to depart} {one time} {there was}\\
\glt \textbf{``Last month, there was a time when an ANA flight was about to depart but there was one more passenger than the number of seats.''}\\
\vspace{-0.1in}
\exi{\textbf{0.8}}
\gll ９日、 この ボランティアに なり   たい 人たちが 集まって、 太田市    で 勉強しました\\ 
      9th   this volunteer      become want people   gather     Ota(city) in  studied \\
\glt \textbf{``On the 9th, people who wanted to become volunteers gathered and studied in Ota.''}\\
\vspace{-0.05in}
\gll 集まった 人たち は、 あと ２回      勉強して テストに 合格する と、 病院     など で 通訳をする ボランティア になります\\
     gathered people {}   more {2 times} study    test     pass     if   hospital like in interpret  volunteer    become\\
\glt \textbf{``The gathered people will become volunteer interpreters in places like hospitals, if they study two more times and pass the test.''}\\
\vspace{-0.1in}
\exi{\textbf{0.7}}
\gll シリア で は、 政府       と  政府       に 反対する 人たち の 戦争 が 続いています\\ 
     Syria  in {}   government and government {} against  people of war  {} {is ongoing}\\
\glt \textbf{``In Syria, the war between the government and the anti-government faction is still ongoing.''}\\
\vspace{-0.05in}
\gll 政府      に 反対する 人たち が たくさん いる       アレッポという町 に は、 政府       の 軍    が ２週間も  空  から 攻撃を 続けています\\
    government {} against  people {} many     {there is} {Aleppo(city)}      in {}   government of army  {} {2 weeks} air from attack maintaining\\
\glt \textbf{``In Aleppo, where there is a large anti-government faction, the government army maintained attacks from the air for two weeks.''}\\
\vspace{-0.1in}
\exi{\textbf{0.6}}
\gll シリア で は、 政府       と  政府       に 反対する 人たち の 戦争 が 続いています\\ 
     Syria  in {}   government and government {} against  people of war  {} {is ongoing}\\
\glt \textbf{``In Syria, the war between the government and the anti-government faction is still ongoing.''}\\
\vspace{-0.05in}
\gll 今  まで  の １０年、    私 は 戦争 が 続いている    所    や 難民    が 生活している 所    へ 何度も               行きました\\
     now until of  {10 years} I  {} war  {}  {is ongoing} place {} refugee {}  {is living} place to {for multiple times} went\\
\glt \textbf{``In the last 10 years, I have made multiple visits to places where a war was ongoing or refugees were living.''}\\
\end{exe}
\end{CJK}
}
\vspace{-0.1in}
\caption{Sample Sentence Pairs in the fuzzy partial orderings with the fuzzy parameter $\alpha=$ 0.9/0.8/0.7/0.6. For each fuzzy parameter $\alpha$, the second sentence is $\alpha$-fuzzily harder than the first sentence. As the fuzzy parameter $\alpha$ decreases, our confidence in the fuzzy partial orderings (the likelihood for a student to understand the first sentence if he/she understands the second one) also drops.  Text source: NHK Easy~\cite{website:nhkeasy}.}
\label{tab:fuzzy_pair}
\end{table*}

==> tab-jrec_4grps.tex <==
\begin{table}[t]
    \minipage{0.48\textwidth}
        \centering
        \begin{tabular}{|c|c|c|}
            Group & Number of Users & Median Number of Texts Read
            \hline
            Adaptive Recommendation & 131 & 13\\
            Assessment & 115 & 12\\
            Recommendation & 91 & 8\\
            Random  & 31 & 8\\
            \hline
        \end{tabular}
        %\vspace{0.1in}
        \caption{Number of Texts Read by Median Users in the Four Groups}
        \label{fig:po_graph}
    \endminipage
    \hfill
    \minipage{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/fuzzypo_edgenum.pdf}
        \vspace{-0.3in}
        \caption{Number of edges in the fuzzy partial ordering graph over different fuzzy parameters, in our corpus of 4,269 texts. Decreasing the fuzzy parameter will increase the graph density exponentially.}
        \label{fig:fuzzy_density}
    \endminipage
    \vspace{-.14in}
\end{table}
